Dual Regularized Optimal Transport

In this paper, we present a new formulation of unbalanced optimal transport called Dual Regularized Optimal Transport (DROT). We argue that regularizing the dual formulation of optimal transport results in a version of unbalanced optimal transport that leads to sparse solutions and that gives us control over mass creation and destruction. We build intuition behind such control and present theoretical properties of the solutions to DROT. We demonstrate that due to recent advances in optimization techniques, we can feasibly solve such a formulation at large scales and present extensive experimental evidence for this formulation and its solution.

==> conclusion.tex <==
%!TEX root = ./full.tex
\section{Conclusion}
\label{sec:conclusion}

In conclusion, in this paper, we present a new formulation of optimal transport called Dual Regularized Optimal Transport. We prove many theoretical results, including connections to the UOT problem, and properties of the solutions for various choices of $\phi, \varphi, \gamma$. We also build the intuition that regularizing $\vf,\vg$ to be more positive results in mass creation and regularizing to be more negative results in mass destruction. We support this intuition with experimental evidence. Finally, we also showed creating mass, via the dual entropic regularized problem results in novel, and useful results when applied to domain transfer. 

We hope that this paper helps understand the dual problem of optimal transport and that future researchers can use the useful interpretations of the dual to design optimal transport based algorithms for their various different applications.  
